Citations and Trust in LLM Generated Responses

Question answering systems are rapidly advancing, but their opaque nature may impact user trust. We explored trust through an anti-monitoring framework, where trust is predicted to be correlated with presence of citations and inversely related to checking citations. We tested this hypothesis with a live question-answering experiment that presented text responses generated using a commercial Chatbot along with varying citations (zero, one, or five), both relevant and random, and recorded if participants checked the citations and their self-reported trust in the generated responses. We found a significant increase in trust when citations were present, a result that held true even when the citations were random; we also found a significant decrease in trust when participants checked the citations. These results highlight the importance of citations in enhancing trust in AI-generated content.

==> images/type_lr.tex <==
\begin{tikzpicture}
\begin{axis}[
    ytick={1,2,3,4,5,6,7,8,9},
    width=4in,
    height=3.5in,
    yticklabels={Question Type, Has Citation, Random Citation, Age Group, Heard of ChatGPT, Education Level, Male, Conservative, Non-White, Urban},
    xlabel={Trust},
    ylabel={},
    ymin = 0.25,
    ymax = 9.75,
    xmax = 0.55,
    xmin = -0.55,
    ]
    \addplot[
    scatter/classes={a={blue}, b={red}, c={green}, d={black}},
    scatter,
    only marks,
    scatter src=explicit symbolic,
    nodes near coords*={\tiny{\sffamily{\Label}}},
    visualization depends on={value \thisrow{label} \as \Label},
    ]%
    plot [error bars/.cd, x dir = both, x explicit, error bar style={very thick ,solid, blue},
      error mark options={line width=0pt,mark size=0pt,rotate=90}]
    table[meta=class, x=x, y=y, x error=ex]{
        y x     ex      class   label
        0.8 0.314 0.156   a      **
        1.8 0.399 0.0906 a   ***
        2.8 -0.263 0.0872 a ***
        3.8 -0.021 0.0336 a  {}
        4.8 0.111 0.1240 a {}
        5.8 -0.044 0.0511 a {}
        6.8 0.082 0.0905 a  {}
        7.8 -0.062 0.0386 a {}
        8.8 0.237 0.0939 a ** 
        9.8 -0.134 0.0698 a * 
    };

        \addplot[
    scatter/classes={a={blue}, b={red}, c={green}, d={black}},
    scatter,
    only marks,
    scatter src=explicit symbolic,
    nodes near coords*={\tiny{\sffamily{\Label}}},
    visualization depends on={value \thisrow{label} \as \Label},
    ]%
    plot [error bars/.cd, x dir = both, x explicit, error bar style={very thick ,solid, red},
      error mark options={line width=0pt,mark size=0pt,rotate=90}]
    table[meta=class, x=x, y=y, x error=ex]{
        y x     ex      class   label
        1.0 0.374 0.0865   b      **
        2.0 0.392 0.0904 b   ***
        3.0 -0.272 0.0869 b ***
        4.0 -0.0187 0.0334 b  {}
        5.0 0.109 0.1240 b {}
        6.0 -0.0364 0.0509 b {}
        7.0 0.0899 0.0903 b  {}
        8.0 -0.0585 0.0385 b {}
        9.0 0.236 0.0937 b ** 
        10.0 -0.133 0.0696 b * 
    };


        \addplot[
    scatter/classes={a={blue}, b={red}, c={green}, d={black}},
    scatter,
    only marks,
    scatter src=explicit symbolic,
    nodes near coords*={\tiny{\sffamily{\Label}}},
    visualization depends on={value \thisrow{label} \as \Label},
    ]%
    plot [error bars/.cd, x dir = both, x explicit, error bar style={very thick ,solid, green},
      error mark options={line width=0pt,mark size=0pt,rotate=90}]
    table[meta=class, x=x, y=y, x error=ex]{
        y x     ex      class   label
        1.2 0.0697 0.275   c      {}
        2.2 0.394 0.0906 c   ***
        3.2 -0.268 0.0872 c ***
        4.2 -0.0175 0.0335 c  {}
        5.2 0.112 0.1240 c {}
        6.2 -0.0406 0.0511 c {}
        7.2 0.0825 0.0906 c  {}
        8.2 -0.0611 0.0387 c {}
        9.2 0.232 0.0940 c ** 
        10.2 -0.132 0.0698 c * 
    };    

\addplot[dashed, samples=50, smooth,domain=0:6, black] coordinates {(0,-1)(0,10)};

\end{axis}
\end{tikzpicture}
